Socially Constructed Treatment Plans: Analyzing Online Peer Interactions to Understand How Patients Navigate Complex Medical Conditions

When faced with complex and uncertain medical conditions (e.g., cancer, mental health conditions, recovery from substance dependency), millions of patients seek online peer support. In this study, we leverage content analysis of online discourse and ethnographic studies with clinicians and patient representatives to characterize how treatment plans for complex conditions are "socially constructed." Specifically, we ground online conversation on medication-assisted recovery treatment to medication guidelines and subsequently surface when and why people deviate from the clinical guidelines. We characterize the implications and effectiveness of socially constructed treatment plans through in-depth interviews with clinical experts. Finally, given the enthusiasm around AI-powered solutions for patient communication, we investigate whether and how socially constructed treatment-related knowledge is reflected in a state-of-the-art large language model (LLM). Leveraging a novel mixed-method approach, this study highlights critical research directions for patient-centered communication in online health communities.

==> Sections/0_Outline.tex <==
\section{Outline}

==> Tables/Contested_posts.tex <==
\begin{table}[t!]
\centering
\renewcommand*{\arraystretch}{1.0}

\begin{tabular}{L{1.5cm}|L{4.5cm}L{5.5cm}L{3cm}}
\textbf{Sub-themes} & \textbf{Guidelines from Authentic Sources}& \textbf{Examples} & \textbf{Comments} \\
\hline
Swallowing 
& 
Suboxone sublingual tablets must be administered whole. Do not cut, chew, or swallow SUBOXONE sublingual tablets. (FDA) & 
I allow Subutex tablets to dissolve under my tongue for as long as possible. However, I often end up swallowing the remainder of the pill. I've read that this might not be the correct method. Can someone explain why this is the case? 
&
The post author partially swallows the pill although guideline prohibits it
\\

\hline
Dosage while tapering 
& 
Do not stop taking SUBOXONE suddenly. You could become sick and have withdrawal symptoms 
& 
I was experiencing severe tooth pain, which is unusual for me, and I observed that my toothache would intensify significantly after each dose. As a result, I reduced my dosage to 8mg 
& 
The post author suddenly stopped taking is medication which contradicts with guidelines\\

\bottomrule
\end{tabular}
\caption{Examples of posts that contradict the authentic guidelines. The examples are paraphrased. }
\label{constested-posts}
\end{table}

==> Tables/Deviated_Strategies.tex <==
\begin{table}[t!]
\centering
\renewcommand*{\arraystretch}{1.0}

\begin{tabular}{L{1.5cm}|L{4.5cm}L{5.5cm}L{3cm}}
\textbf{Topic} & \textbf{Guidelines from Authentic Sources}& \textbf{Examples} & \textbf{Comments} \\
% Taking alcohol & You should not drink alcohol or take prescription or over-the-counter medicines that contain alcohol while taking SUBOXONE sublingual film, because this can lead to loss of consciousness or even death. & Try a few drops of clear/unflavored alcohol like vodka or try brushing your teeth and using an alcohol-based mouthwash before you put it under your tongue. Good luck & \\
% \hline
% Snorting & Do not inject (“shoot-up”) or snort SUBOXONE sublingual tablet. (Source: FDA) & Start with half of a quarter. I personally snort them and find that it works better than sublingual. I'm talking about the 8mg pills by the way. You're safe to go ahead and take it now. & Although snorting is prohibited in the guidelines, peer is suggesting to snort.\\
\hline
Swallowing & Suboxone sublingual tablets must be administered whole. Do not cut, chew, or swallow SUBOXONE sublingual tablets. (FDA) & I swallow mine because that way whatever you don’t absorb sublingually will slowly absorb through the stomach. & Peer suggests swallowing while the guideline prohibits it. \\
% \hline
% Between Treatment Types & Patients switching from methadone to buprenorphine in the treatment of OUD should be on low doses of methadone prior to switching medications. & Coming from subs and not in active addiction, we should be able to use lower doses of methadone. I’m hoping for 40-60mg. It’s also reversible; you can go back to subs, but you’ll need like a week to manage the transition whereas it’s easy to go from subs to methadone. & \\
% \hline
% Waiting time to resume MOUD & During induction, generally, buprenorphine initiation should occur at least 6–12 hours after the last use of heroin or other short-acting opioids, or 24–72 hours after their last use of long-acting opioids such as methadone. (Source: ASAM) & When you think you feel shitty, keep waiting. Trust me. I would go at least 5 days. I wish you the best. & \\
\hline
Dosage while tapering & Do not stop taking SUBOXONE suddenly. You could become sick and have withdrawal symptoms &  If you were only taking 30mg a day, I would say do a rapid Suboxone detox and 2mg should be more than enough. & Peer is suggesting rapid detox which contradicts with guidelines\\
% \hline
% Cutting tablets/strips & Take the entire SUBOXONE sublingual film. Do not cut, tear, chew, or swallow SUBOXONE sublingual film because the medicine will not work as well. & Not personally. But I’ve seen some reports here about it. They are acidic and can cause gum and bone damage, so I’d imagine it’s definitely possible. Doesn’t seem like something to run to the doctor for yet. It’s best to take them bucally and change the placement every time you take them. I also suggest cutting them in half and using 2 different spots at one time, not only for less irritation in one area but also for better absorption. & \\
\bottomrule
\end{tabular}
\caption{Examples of strategies suggested by peers deviate from authentic guidelines. The examples are paraphrased. }
\label{peer-suggestions-deviations}
\end{table}

==> Tables/Full_Table.tex <==
\begin{landscape}
\begin{table}[ht]
\centering
\begin{tabular}{|p{1.75cm}|p{1.25cm}|p{3cm}|p{3cm}|p{3cm}|p{5.5cm}|}
\hline
\textbf{Branches} & \textbf{Topics} & \textbf{Guidelines} & \textbf{Issues} & \textbf{Example Post (Paraphrased)} & \textbf{Summarized Strategy List (by peers)} \\ \hline
\multirow{2}{1.5cm} {Route of administration} & Dissolving under the tongue & 
\begin{itemize}[leftmargin=0.25cm, topsep=0pt]
    \item While SUBOXONE sublingual film is dissolving, do not chew or swallow the film because the medicine will not work as well. 
    \item After SUBOXONE is completely dissolved, rinse your mouth with water and swallow. Wait for at least one hour before brushing teeth.
    \item Advise patients not to eat or drink anything until the tablet is completely dissolved.
\end{itemize}
& 
\begin{itemize}[leftmargin=0.25cm, topsep= 0pt]
    \item Bupe not dissolving under the tongue 
    \item dissolving under the tongue is giving nosebleeds
    \item how to dissolve
    \item Dissolving issue- too slowly/too quickly
    \item How to absorb the residual saliva 
\end{itemize}
 & 
 Bupe is not dissolving under the tongue \newline
 Bupe is supposed to dissolve under the tongue in about 10 minutes, am I right? For some reason, mine just won't dissolve. I've had them under my tongue for 25 minutes now, and they're still the same. Any Suggestions?
 &

 % Peers provided various suggestions for optimizing the absorption of sublingual buprenorphine (bupe) for opioid use disorder treatment. Key recommendations include:
 \begin{enumerate}[leftmargin=0.5cm, topsep=0pt]
     \item **Dissolution Time**: Allow the medication to dissolve for 20-60 minutes, with some suggesting up to an hour for better absorption.
     \item **Minimize Saliva**: Reduce saliva in the mouth to enhance absorption; avoid swishing or swallowing the medication.
     \item **Crushing Pills**: Consider crushing the pill and placing the powder under the tongue to improve absorption.
     
     \item **Positioning**: Leaning forward or looking down while taking the medication may help.
     \item **Alternative Placement**: Placing the medication between the gum and cheek can allow for gradual absorption.
     \item **Pre-treatment**: Using a small amount of alcohol or brushing teeth before taking bupe may aid in dissolution.
     \item **Personal Experience**: Some users prefer strips over tablets due to faster dissolution times.
\end{enumerate}
% Overall, these strategies aim to maximize the effectiveness of buprenorphine treatment while minimizing wasted doses.
 \\ \cline{2-6} 

&
Swallowing
& 
\begin{itemize}[leftmargin=0.25cm, topsep=0pt]
    \item SUBOXONE sublingual tablets must be administered whole. Do not cut, chew, or swallow SUBOXONE sublingual tablets.
    \item Do not to eat or drink anything until the tablet is completely dissolved.
\end{itemize}
& 
\begin{itemize}[leftmargin=0.25cm, topsep=0pt]
    \item Question about whether to swallow
    \item Question on how to swallow 
    \item Swallowed opioids while on MOUD treatment
    \item Curious whether a side-effect (e.g., headache) is due to swallowing subs
    \item Discussing the effect of swallowing
\end{itemize}
& 
Need help with dosing \newline
Here are my questions: What’s the appropriate starting dose for this medication? How frequently should I take it? What’s the correct way to take it—do I swallow the pills? I think I read that you place them under your tongue—is that correct? 
% Someone gave me 2mg and 8mg pills. Is that the right amount, or is it too much or too little? How long after my last dose of Percocet should I take this? It’s been 18 hours since my last Percocet dose, and I’m feeling terrible. It’s only going to get worse, right?
& 
% In response to questions about starting doses for opioid use disorder treatment with Suboxone, peers provided various suggestions. The consensus is to begin with a low dose, typically around 2mg, and adjust as needed. Some recommend sublingual administration, while one peer suggests snorting for better effects. It's advised to wait an hour before redosing and to avoid taking too much to prevent sickness. A rapid detox approach is also mentioned for those transitioning from lower doses of opioids. Overall, the emphasis is on careful dosing and personal adjustment to find what works best. 

% **Suggestions:**
 \begin{enumerate}[leftmargin=0.5cm, topsep=0pt]
    \item Start with 2mg sublingually.
    \item Hold the liquid under the tongue for 10 minutes before swallowing.
    \item Wait an hour before considering a second dose.
    \item Avoid exceeding 4mg daily.
    \item Some suggest snorting the medication for better effects.
    \item Consider a rapid Suboxone detox if transitioning from lower opioid doses.
\end{enumerate}
\\ \hline





% Add more rows as needed
\end{tabular}
\caption{Table Caption (TBD)}
\label{tab:Full_Table}
\end{table}
\end{landscape}

% \begin{itemize}[leftmargin=0.25cm, topsep=0pt]
%     \item 
%     \item
%     \item 
% \end{itemize}
